DIPS: Optimal Dynamic Index for Poisson $\boldsymbol{\pi}$ps Sampling

This paper addresses the Poisson $\pi$ps sampling problem, a topic of significant academic interest in various domains and with practical data mining applications, such as influence maximization. The problem includes a set $\mathcal{S}$ of $n$ elements, where each element $v$ is assigned a weight $w(v)$ reflecting its importance. The goal is to generate a random subset $X$ of $\mathcal{S}$, where each element $v \in \mathcal{S}$ is included in $X$ independently with probability $\frac{c\cdot w(v)}{\sum_{v \in \mathcal{S}} w(v)}$, where $0<c\leq 1$ is a constant. The subsets must be independent across different queries. While the Poisson $\pi$ps sampling problem can be reduced to the well-studied subset sampling problem, updates in Poisson $\pi$ps sampling, such as adding a new element or removing an element, would cause the probabilities of all $n$ elements to change in the corresponding subset sampling problem, making this approach impractical for dynamic scenarios. To address this, we propose a dynamic index specifically tailored for the Poisson $\pi$ps sampling problem, supporting optimal expected $\mathcal{O}(1)$ query time and $\mathcal{O}(1)$ index update time, with an optimal $\mathcal{O}(n)$ space cost. Our solution involves recursively partitioning the set by weights and ultimately using table lookup. The core of our solution lies in addressing the challenges posed by weight explosion and correlations between elements. Empirical evaluations demonstrate that our approach achieves significant speedups in update time while maintaining consistently competitive query time compared to the subset-sampling-based methods.

==> lemmas/em_geo.tex <==
\begin{lemma}[jump solution for bounded probability in \emph{EM}]\label{em_grs} {
    Given a \emph{subset sampling} problem instance $\Psi=\left<\S, \bp\right>$, if $\bp(\S)\subseteq(\bar{p}/2, \bar{p}]$, where $\bar{p}\in(0,1]$, then there is a data structure $\D$ of $\bigo{n/B}$ space that answers a query in $\Bigo{(\mu_\S/B)\log_{M/B} (n/B)}$ amortized expected I/Os.
} \end{lemma}

% \begin{proof} 
% The data structure and the query method are as follows.

% \header{\bf Structure.}
% We use the set sampling structure in~\cite{irs} to store $\S$.

% \header{\bf Query.}
% We first overestimate the probability of each $v\in\S$ as $\bar{p}$. Then we keep drawing random number $g_i$ from $\geo{\bar{p}}$ ($i=1,2,\ldots$). Let $t$ be the smallest number such that $\sum_{i=1}^{t+1} g_i\geq n$. We stop drawing random numbers immediately after $g_{t+1}$ is drawn. 
% %then we have decided to sample $t$ elements from $\S$.
% Notice that this process can be done in memory with no extra I/Os. 
% % Recap that $X$ denote the random subset returned by a \emph{subset sampling} query. We next make an critical observation that, conditioned on $\norm{X}=t$, the probability that $X=T$ is identical for each subset $T\subseteq\S$. More precisely, we have 
% % $$\Pr[X=T\subseteq\S\mid\norm{X}=t]=\frac{\bar{p}^t(1-\bar{p})^{n-t}}{\tbinom{n}{t}\bar{p}^t(1-\bar{p})^{n-t}}=\frac{1}{\tbinom{n}{t}}$$.
% Then we initiate a \emph{without replacement} query with parameter $t$ to the set sampling structure. Let $Z$ denote the random subset returned by the set sampling structure. We define $\bar{\bp}(v)=\bar{p}$ for $v\in\S$. Recap that $t\sim Binomial(n,\bar{p})$. Then we have
% \begin{align*}
% \Pr[Z=T\subseteq\S]&=\Pr[t=\norm{T}]\cdot\Pr[Z=T\mid t=\norm{T}]\\
% &=\tbinom{n}{\norm{T}}\bar{p}^{\norm{T}}(1-\bar{p})^{n-\norm{T}}\cdot\frac{1}{\tbinom{n}{\norm{T}}}\\
% &=\bar{p}^{\norm{T}}(1-\bar{p})^{n-\norm{T}}\\
% &=\left( \prod_{v\in T}\bar{\bp}(v) \right)\left( \prod_{v\in {\S\setminus T}}(1-\bar{\bp}(v)) \right).
% \end{align*}
% Thus $Z$ can be regarded as a query result from \emph{subset sampling} problem instance $\left<\S, \bar{\bp}\right>$.

% Since the elements in $Z$ are sampled with overestimated probability, we need to scan across $Z$ and draw a random number $u$ from $\unif{0}{\bar{p}}$ for each $v\in Z$. If $u<\pv$, we keep $u$, otherwise we discard $u$. After this checking process, we finally get a valid result for \emph{subset sampling} query on $\Psi$.

% Recap that the expectation of $t$ is $E[t]=n\times\bar{p}\leq\sum_{v\in\S}2\pv=2\mu_\S$, so the amortized expected query time is:
% $$E[t]\Bigo{(1/B)\log_{M/B} (n/B)}=\Bigo{(\mu_\S/B)\log_{M/B} (n/B)}.$$
% \end{proof}


==> lemmas/em_naive.tex <==
\begin{lemma} [naive solution in EM] \label{em_naive} 
    Given a \emph{subset sampling} problem instance $\Psi=\left<\S, \bp\right>$, there is a data structure $\D$ of $\bigo{n/B}$ space that answers a query in $\bigo{n/B}$ amortized expected I/Os.
\end{lemma}
\begin{proof}
    Since the naive solution only involves array scanning, the space and query time under the \emph{EM} model are that of the \emph{Real RAM} model divided by $B$.
\end{proof}


==> lemmas/em_reduce.tex <==
\begin{lemma}[size reduction in \emph{EM}] \label{em_sr}
Given a \emph{subset sampling} problem instance $\Psi=\left<\S, \bp\right>$, assume that using method $\mathcal{M}$, for the \emph{subset sampling} problem instance $\widetilde\Psi=\left<\smS, \sbp\right>$, there is a data structure $\widetilde{\D}$ of $\bigo{s_0}$ space that answers a query in $\bigo{t_0}$ I/Os, then for the \emph{subset sampling} problem instance $\Psi$, there is a data structure $\mD$ of $\bigo{s_0+|\S|/B}$ space that answers a query in $\bigo{t_0+1/B+(\mu_\S/B)\log_{M/B} (\norm{\S}/B)}$ amortized expected I/Os.
\end{lemma}

% \begin{proof}
%     The data structure and the query method are as follows.

%     \header{\bf Structure.}
%         We now maintain a data structure $\D_{L^+}$ for $\left<\S_{\twologtwo^+}, \frac{\restr{\bp}{\S_{\twologtwo^+}}}{\widetilde\bp(\twologtwo)}\right>$ using Lemma \ref{em_naive} (naive solution in \emph{EM}), maintain data structure $\D_l$ for $\left<\S_l, \frac{\restr{\bp}{\S_l}}{\widetilde\bp(l)}\right>$ using Lemma \ref{em_grs} for $1\leq l\leq\twologone$. Finally we maintain a data structure $\widetilde{\D}$ for $\widetilde\Psi$ using $\mathcal{M}$. Since we focus on static structure in \emph{EM} and we don't need to support dynamic operation in this case, $\frac{\bp}{\widetilde\bp(l)}$ ($1\leq l\leq\twologtwo$) can be stored explicitly. The total space used is $\bigo{s_0}+\bigo{\norm{\S}}=\bigo{s_0+\norm{\S}}$.
    
%     \header{\bf Query.}
%         The steps for answering the query are the same as that of Lemma \ref{sr}. The amortized expected time complexity:
%         \begin{align*}
%         &\bigo{t_0}+\sbpo{\twologtwo} \Bigo{\left|\S_{\twologtwo^+}\right|/B}+\sum_{l=1}^{\twologone}\sbpo{l}\Bigo{\left(\frac{\mu_{\S_l}}{\sbpo{l}B}\right)\log_{M/B} (n/B)} \\
%         &\leq\quad \bigo{t_0}+\frac{|\S|}{|\S|^2}\bigo{|\S|/B}+\sum_{l=1}^{\twologone}\Bigo{(\mu_{\S_l}/B)\log_{M/B} (n/B)} \\
%         &=\quad \bigo{t_0}+\bigo{1/B}+\Bigo{(\mu_\S/B)\log_{M/B} (n/B)}\\
%         &=\quad \Bigo{t_0+1/B+(\mu_\S/B)\log_{M/B} (n/B)}.
%         \end{align*}
% \end{proof}


==> lemmas/geo.tex <==
\begin{lemma}[jump solution for bounded probability]\label{grs} {
    Given a \emph{subset sampling} problem instance $\Psi=\left<\S, \bp\right>$, if $\bp(\S)\subseteq(\bar{p}/2, \bar{p}]$, where $\bar{p}\in(0,1]$, then we can maintain a data structure $\D$ of size $\bigon$ with $\bigomu$
    expected $\que$ time. Furthermore, $\D$ can be maintained with $\bigone$ $\upd$ time, $\bigone$ amortized expected $\ins$ and $\del$ time. 
} \end{lemma}

% \begin{proof} The data structure and modification operations can be handled similar to Lemma \ref{naive}.

%     We answer the \emph{subset sampling} query as follows. We first overestimate the probability of each $v\in\S$ as $\bar{p}$. When the probabilities are all equal to $\bar{p}$, we can quickly sample a subset $\bar{X}$ by repeatedly drawing a random number $g$ from $\geo{\bar{p}}$ and then jump to the next $g$ position, and include the element at this position in $\bar{X}$. We keep jumping until we reach the end of the array $A$. Because we may grant $v\in\bar{X}$ with extra probability, we should draw a number $u$ from $\unif{0}{\bar{p}}$ and finally include $v$ in $X$ if and only if $u\leq\pv$. In this way, each element $v\in\S$ is sampled into $X$ with probability $\bar{p}\times\frac{\pv}{\bar{p}}=\pv$. 

%     We next analyze the query time.
%     Let $g_1, g_2, \ldots$ be the sequence of random number we generate during the above process. Let $t$ be the smallest number such that $\sum_{i=1}^{t+1} g_i\geq n$. On the one hand, $t$ can be interpreted as the number of jumps before reaching the end. On the other hand, $t$ can be interpreted as the number of success trails among $n$ independent trails each with success probability $\bar{p}$. We can take the later interpretation and derive that $t\sim\bin{n}{\bar{p}}$. The expected number of jumps is thus $E[t]=n\bar{p}\leq\sum_{v\in\S}2\pv=2\mu_\S$. So the expected query time is $\bigo{1+\mu_\S}$.
% \end{proof}


==> lemmas/lookup.tex <==
    % table lookup

    \begin{lemma}[table lookup]\label{lookup}
    Given a \emph{subset sampling} problem instance $\Psi^o= \left< \S^o, \textbf{p}^o \right>$, where $\S^o=\setht{1,2}{m}$ and the \emph{codomain} of function $\textbf{p}^o$ is $\setht{\frac{0}{m^2}, \frac{1}{m^2}}{\frac{m^2-1}{m^2}, \frac{m^2}{m^2}}$,  we can maintain a data structure $\mD^o$ of size $m^{\bigo{m}}$ with $\bigo{1+\mu_{\S^o}}$ expected $\que$ time. Furthermore, $\mD^o$ can be maintained with $\bigone$ $\upd$ time.
    \end{lemma}

    Note that we assume discretized probability here for the ease of tabulation. We will show how to discretize in Theorem \ref{sampling structure}. Let us first see an example before delving into the proof.
     \begin{example}
     Suppose $\S^o=\{1,2,3,4\}$, let us discuss what we should pre-compute for a specific status of $\bp^o$, say $\bp^o(1)=\frac{3}{16}$, $\bp^o(2)=\frac{7}{16}$, $\bp^o(3)=\frac{4}{16}$, $\bp^o(4)=\frac{5}{16}$. Let $p_{i,j}$ be the entry in the $(i+1)$-th row and $(j+1)$-th column of Table \ref{tab:conceptual}. Then $p_{i,j}$ represents the probability that the last sampled element is $i-1$ and the next successfully sampled element is  $j$. Note that element $0$ and $m+1$ are sentinel values. ``The last sampled element is $0$'' stand for the start of the jump process. ``The next successfully sampled element is $m+1$'' stands for the fact that $i,i+1,\dots,m$ are all not sampled. Conceptually, we can draw a random number $u$ from $\unif{0}{1}$, and find the unique $j\in\setht{i,i+1}{m,m+1}$ with $\sum_{k=i}^{j-1}p_{i,k}<u\leq\sum_{k=i}^{j}p_{i,k}$ and decide to jump to $j$ on the fly, which costs $\bigo{m}$ time and is costly. To avoid such expensive online cost, we encode such information with a pre-computed array for $j$ such that it considers all possible statuses of generated random numbers. Observe that after multiplying $p_{i,i},p_{i,i+1},\dots,p_{i,m+1}$ by their lowest common denominator, which is $(m^2)^{m-i+1}$, it suffice to draw a random integer $du$ from $[1,(m^2)^{m-i+1}]$, for deciding where to jump to. Then for fixed $\bp^o$ and $i$, we can easily pre-compute an array of size $(m^2)^{m-i+1}$, where the $k$-th entry of the array stores the unique $j$ we should jump to if the generated random integer $du=k$. We show the array pre-computed for the above $\bp^o$ and $i=2$ in Table \ref{tab:array_2}, the array pre-computed for the above $\bp^o$ and $i=3$ in Table \ref{tab:array_3}.
     \end{example}

     Next, we are ready to give the detailed proof.
    \begin{proof} 
    The data structure, query operation, and update operation are as follows.
        \input{tables/conceptual}
     \input{tables/array_2}
     \input{tables/array_3}   
    \header{\bf Structure.}
    We use a numeral system with radix $m^2+1$ to encode $\textbf{p}^o$, i.e. we represent $\textbf{p}^o$ as: 
    $$\lambda=\left(\left(m^2p^o(m)\right)\ \left(m^2p^o(m-1)\right)\dots\left(m^2p^o(2)\right)\left(m^2p^o(1)\right)\right)_{m^2+1} .$$ 
    Then there are $(m^2+1)^m$ possible statuses of $\textbf{p}^o$, i.e., each number in the numeral system with radix $m^2+1$ indicates a status. For a fixed $\textbf{p}^o$, we calculate 
    $$\beta[\lambda][i]=m^2p^o(i), \overline{\beta}[\lambda][i]=m^2(1-p^o(i)),$$ 
    for $i\in[1,m]$. We set $\beta[\lambda][m+1] = 1$. For each $1\leq i\leq j\leq m$, we pre-compute the integers $Mass[\lambda][i][j]$ that are proportional to the probability that the last sampled element is $i-1$ and the next successfully sampled element is  $j$. 
    Note that when $i=1$, ``the last sampled element is $0$''  stands for the start of the sampling process. 
    We also pre-compute $Mass[\lambda][i][m+1]$, which is proportional to the probability that the elements $i,i+1\ldots,m$ are all not sampled. This is done by calculating 
    $$Mass[\lambda][i][j]=\left(\prod_{k=i}^{j-1}\overline{\beta}[\lambda][k]\right)\beta[\lambda][j](m^2)^{\max{0}{m-j}}$$ 
    for $j\in[i+1,m+1]$ and calculating 
    $$Mass[\lambda][i][i]=\beta[\lambda][i](m^2)^{\max{0}{m-i}}.$$ 
    Next, we maintain an array of size $(m^2)^{m-i+1}$ at $Tb[\lambda][i]$. For each $1\leq r\leq{(m^2)^{m-i+1}}$, we fill in $Tb[\lambda][i][r]$ with the unique $j\in\setht{i,i+1}{m,m+1}$ with 
    $$\sum_{k=i}^{j-1}Mass[\lambda][k]<r\leq\sum_{k=i}^{j}Mass[\lambda][k]$$
    in $\mathcal{O}(m)$ time. The total space is thus 
    $$(m^2+1)^m\times m \times m^{\bigo{2m}}=m^{\bigo{m}}.$$ 
    Since each entry can be computed in $\bigo{m}$ time, the initialization time is also $m^{\bigo{m}}$.
    
    \header{\bf Query.}
    For the \emph{subset sampling} query, we start with $i=1$ and draw a random integer $du$ from $[1,(m^2)^{m-i+1}]$. Then, we check the table and access the array stored at table entry $Tb[\lambda][i]$ to determine the next successfully sampled element, suppose $Tb[\lambda][i][du]=j$, then we set $i=j$. This process continues until $m+1$ is sampled, and the expected time complexity is $\Bigo{1+\sum_{v\in\S^o}\pv}=\bigo{1+\mu_{\S^o}}$. According to the construction of the lookup table, each element $v\in\S^o$ is sampled into with correct probability $\bp^o(v)$.
    
    \header{\bf Update.}
     For $\updtwo{v}{p}$ operation, it is equivalent to updating the $v$-th digit of the $(m^2+1)$-based number $\lambda$, which is a generalized \emph{bit operation}. Specifically, we update $\lambda$ to $$\lfloor\frac{\lambda}{(m^2+1)^v}\rfloor(m^2+1)^v+(m^2p)(m^2+1)^{v-1}+\lambda\%(m^2+1)^{v-1},$$ which can be done in $\bigone$ time.
    \end{proof}

==> lemmas/naive.tex <==
\begin{lemma} [naive solution] \label{naive} 
    Given a \emph{subset sampling} problem instance $\Psi=\left<\S, \bp\right>$, we can maintain a data structure $\D$ of size $\bigon$ with $\bigon$ $\que$ time. Besides, $\D$ can be maintained with $\bigone$ $\upd$ time, $\bigone$ amortized expected $\ins$ and $\del$ time.
\end{lemma}
% \begin{proof}
% We can achieve the claimed \emph{update}, \emph{insert} and \emph{delete} time by maintaining a dynamic array $A$ in arbitrary order and a hash table to map from each element $v\in\S$ to its location in array $A$. We further maintain the size $n$ of $\S$. To answer query, for each $j\in\setht{1,2}{n}$, we draw a random number $u_j$ from $\unif{0}{1}$. If $u_j < \bp(A[j])$, we include $A[j]$ in $X$. Since every element is examined once, the query time is thus $\bigon$.
% \end{proof}

==> lemmas/reduce.tex <==

We define $\S_l=\{v|v\in\S,2^{-l}<\pv\leq2^{-l+1}\}(l\in\integer^+)$. Readers can interpret $\S_{l}$ as the bucket which stores elements whose sampling probabilities fall in the range $(2^{-l},2^{-l+1}]$. 

Furthermore, we define $\S_{l^+}=\cup_{i\geq l}\S_i$. Readers can interpret $\S_{l^+}$ as the bucket which stores elements whose sampling probabilities are less than or equal to $2^{-l+1}$.

Let $Q$ be a subset of $\S$. We define a function $\bq_\bp:\P(\S)\to[0,1]$, where $\P(\S)$ is the power set of $\S$ and $\bq_\bp(Q)=\Pr[$at least one element in $Q$ is sampled$]=1-\prod_{v\in Q}(1-\pv)$. According to the union bound, we have $\bq_\bp(Q)\leq\min{1}{\sum_{v\in Q}\pv}= \min{1}{\mu_Q}$.
        
We define $L=2\lc\log|\S|\rc+2$, which is the number of buckets we will maintain in the Lemma \ref{sr}. We define $\widetilde{\S}=\{1,2,...,L\}$, which is the index set for the buckets. We then define 
$$\widetilde{\bp}(i)=
    \left\{
    \begin{aligned}
    &\bq_\bp(\S_i),1\leq i\leq L-1 \\
    &\bq_\bp(\S_{i^+}) ,i = L
    \end{aligned}\right. 
,$$
which assigns the sampling probability for each bucket.


Then, in Appendix~\ref{pf_sr}, we prove the following lemma:

\begin{lemma}[size reduction] \label{sr}
Given a \emph{subset sampling} problem instance $\Psi=\left<\S, \bp\right>$, 
    assume that using method $\mathcal{M}$, for the \emph{subset sampling} problem instance $\widetilde\Psi=\left<\smS, \sbp\right>$, we can maintain a data structure $\widetilde{\D}$ of size $\bigo{s_0}$ with $\bigo{t_0}$ $\que$ time and $\bigone$ amortized expected $\upd$ time. Then for the \emph{subset sampling} problem instance $\Psi$, we can maintain a data structure $\mD$ of size $\bigo{s_0+|\S|}$ with $\bigo{t_0+1+\mu_\S}$ expected $\que$ time and $\bigone$ amortized expected $\upd$, $\ins$ and $\del$ time.
\end{lemma}
% \begin{proof}
%     %Recap that for a subset $A$ of the domain of $\bp$, $\restr{\bp}{A}$ represents the \emph{restriction} of $\bp$ to $A$. 
%     The data structure, query operation and modification operations are as follows.

%     \header{\bf Structure.}
%         % Because $\Pr$[at least one element $v\in\S_{\twologtwo^+}$ is sampled$]\leq\frac{1}{2^{-L+1}}\times \norm{\S_{L^+}}\leq\frac{1}{\norm{\S}^2}\times \norm{\S}=\frac{1}{\norm{\S}}$ according to the union bound, we can maintain a data structure $\D_{L^+}$ for $\left<\S_{\twologtwo^+}, \frac{\restr{\bp}{\S_{\twologtwo^+}}}{\widetilde\bp(\twologtwo)}\right>$ using Lemma \ref{naive} (naive solution) without worrying about degrading the overall query time. 
%         We maintain a data structure $\D_{L^+}$ for $\left<\S_{\twologtwo^+}, \frac{\restr{\bp}{\S_{\twologtwo^+}}}{\widetilde\bp(\twologtwo)}\right>$ using Lemma \ref{naive} (naive solution).
%         Here, $\restr{\bp}{\S_{\twologtwo^+}}$ indicates the \emph{restriction} of function $\bp$ to $\S_{\twologtwo^+}$. 
%         It is defined for the consistency of the definition of a \emph{subset sampling} problem instance. 
%         We maintain data structure $\D_l$ for $\left<\S_l, \frac{\restr{\bp}{\S_l}}{\widetilde\bp(l)}\right>$ using Lemma \ref{grs} (jump solution for bounded probability) for $1\leq l\leq\twologone$. Finally we maintain a data structure $\widetilde{D}$ for $\widetilde\Psi$ using $\mathcal{M}$.
%         Note that we store $\bp$ and $\widetilde\bp(l)$ separately instead of storing $\frac{\bp}{\widetilde\bp(l)}$ explicitly for $1\leq l\leq\twologtwo$.
%         %It should be noted that during the initialization of the data structure for each subproblem, the size of the dynamically allocated array should be twice that of the subproblem. 
%         We also record the size of $\S$ when we first initialize the data structure in $OldSize$ and record the current size of $\S$ in $Size$. 
%         %We will compare $OldSize$ and $Size$ to decide when to rebuild the whole structure. 
%         The total space used is $\bigo{s_0}+\bigo{\norm{\S}}=\bigo{s_0+\norm{\S}}$.
    
%     \header{\bf Query.}
%         For \emph{subset sampling} query, we first draw an index set $\sX$ from $\widetilde{\S}$ using $\widetilde{\D}$. Then we draw $X_l$ from bucket $S_l$ using $\D_l$ for each $l\in\sX\setminus\{\twologtwo\}$ and draw $X_{l}$ from bucket $\S_{\twologtwo^+}$ using $\D_{l^+}$ for each $l\in\sX\cap\{\twologtwo\}$. Finally we return $X=\cup_{l\in\sX}X_l$. 
%         The expected time complexity is:
%         \begin{align*}
%         &\bigo{t_0}+\sbpo{\twologtwo} \Bigo{\left|\S_{\twologtwo^+}\right|}+\sum_{l=1}^{\twologone}\sbpo{l}\Bigo{1+\frac{\mul}{\sbpo{l}}} \\
%         &\leq\quad \bigo{t_0}+\frac{|\S|}{|\S|^2}\mathcal{O}(|\S|)+\sum_{l=1}^{\twologone}\sbpo{l}+\sum_{l=1}^{\twologone}\bigo{\mul} \\
%         &=\quad \bigo{t_0}+\bigone+\mathcal{O}(\mu_\S)+\mathcal{O}(\mu_\S) \\
%         &=\quad \bigo{t_0+1+\mu_\S}.
%         \end{align*}
%         In this way, each element $v\in\S_l$ for $1\leq l\leq\twologone$ is sampled into $X$ with probability $\sbpo{l}\times\frac{\pv}{\sbpo{l}}=\pv$. Each element $v\in\S_{\twologtwo^+}$ is sampled into $X$ with probability $\sbpo{\twologtwo}\times\frac{\pv}{\sbpo{\twologtwo}}=\pv$.
    
%     \header{\bf Modification.}
%         % The description and analysis of the modification operations are deferred to Appendix \ref{modif}.
%         %%%%%%%%%%
%         % update %
%         %%%%%%%%%%
%         For $\updtwo{v}{p}$ operation, we first locate the $\S_l$ which contains $v$ and the $\S_{l^\prime}$ which would contain $v$ after update. This can be done in $\bigo{1}$ time by calculating 
%         $$l=\min{-\lf\log \pv\rf}{\twologtwo}, l^{\prime}=\min{-\lf\log p\rf}{\twologtwo}.$$
%         If $l\neq l^\prime$, then we delete $v$ from $\S_l$, insert $v$ into in $\S_{l^\prime}$, and update $\sbpo{l}$ and $\sbpo{l^\prime}$ accordingly. Otherwise, we simply do an update operation in $\S_l=\S_{l^\prime}$ and update $\sbpo{l}$ accordingly. In both cases, the time complexity is amortized expected $\bigo{1}$.
%         %%%%%%%%%%
%         % insert %
%         %%%%%%%%%%
        
%         For $\instwo{v}{p}$ operation, we first increment $Size$ by one and augment $\bp$ with $\pv=p$. 
%         If $Size<2\times OldSize$, then we locate the $\S_l$ which would contain $v$, insert $v$ into $\S_l$ and update $\sbpo{l}$ accordingly. In this case, the time complexity is amortized expected $\bigo{1}$. If $Size=2\times OldSize$, we reconstruct the whole data structure. As an overflow reconstruction happens after at least $\bigo{|\S|}$ insert operations, and the reconstruction time is $\bigo{|\S|}$, thus in this case the time complexity is also amortized expected $\bigo{1}$.

        
%         %The steps and analysis for $\delone{v}$ are analogous to $\instwo{v}{p}$ operation.
%         For $\delone{v}$ operation, we first decrement $Size$ by one and remove $\pv$.
%         If $Size>\frac{OldSize}{2}$, then we locate the $\S_l$ which contains $v$, delete $v$ from $\S_l$ and update $\sbpo{l}$ accordingly. In this case the time complexity is amortized expected $\bigo{1}$. If $Size=\frac{OldSize}{2}$, we reconstruct the whole data structure. As an underflow reconstruction happens after at least $\bigo{|\S|}$ delete operations, and the reconstruction time is $\bigo{|\S|}$, thus in this case the time complexity is also amortized expected $\bigo{1}$. 
% \end{proof}


==> lemmas/rssp2_baseline.tex <==

\header{\bf Structure.}
There are mainly three steps in building our data structure.
\begin{enumerate}
    \item We first build a treap $\T$ on $\S$, for each node $u$ in $\T$, we associate it with a probability $\bq_\bp(Leaves(u))$ and a \textit{dynamic subset sampling} structure $\mA(u)$ using Theorem \ref{sampling structure} on $Leaves(u)$. Note that the sampling probability for each $\v\in Leaves(u)$ is set as $\frac{\pv}{\bq_\bp(Leaves(u))}$. The space consumption for all $A(u)$ adds up to $\bigonlog$. Then, consider a $\iconc$ leaf node $v$, for each node $u$ on the search path to $v$, we associate it with a \textit{dynamic subset sampling} structure $\mA(\Ruv)$ (resp. $\mA(\Luv)$) using Theorem \ref{sampling structure} for $\Ruv$ (resp. $\Luv$). Since there are $\bigon$ $\iconc$ leaves, each search path to leaf is of length $\bigolog$, and each $\Ruv$ or $\Luv$ consists of $\bigolog$ nodes, the space consumption for all $\Luv$ and $\Ruv$ adds up to $\bigo{n\log^2 n}$. Thus the total space usage of step 1 is $\bigo{n\log^2 n}$.
    
    \item We build a $\VEBT$ that can return $pre(a)$ and $suc(a)$ of an integer $a\in[U]$ using $\bigologlogu$ time. The space consumption of this structure is $\bigon$.

    \item We build a \textit{dynamic lowest common ancestor (LCA) structure} that can return the lowest common ancestor of any two leaves of $\T$ in $\bigone$ time. The space consumption of this structure is $\bigon$. It can support insertion or deletion with $\bigone$ time.
\end{enumerate}
The total space consumption of our data structure is $\bigo{n\log^2 n}$.

\header{\bf Query.}
Given input range $[a,b]$ at query time, we first locate $pre(a)$ and $suc(b)$ in $\bigologlogu$ time. Then, we use the $\DLCA$ to locate $u$, the lowest common ancestor of $pre(a)$ and $suc(b)$ in $\bigone$ time. We know that $\mathcal{R}(u, pre(a))\cup\mathcal{L}(u,suc(b))$ forms the canonical nodes $\mC(a,b)$ of $[a,b]$. Instead of sampling from these $\bigolog$ canonical nodes one by one, we now first sample a subset $\mC$ from the canonical nodes using $\mA(\mathcal{R}(u, pre(a)))$ and $\mA(\mathcal{L}(u,suc(b)))$. Then for each $c\in \mC$, we use $\mA(c)$ to sample a subset from $Leaves(c)$ and finally return the union of these subsets. The expected time is:
        \begin{align*}
        &\bigologlogu+\bigone+\sum_{c\in\mC(a,b)}\bq_\bp(Leaves(c))\mathcal{O}(1+\frac{\mu_{Leaves(c)}}{\bq_\bp(Leaves(c))})\\
        =\quad&\bigologlogu+\sum_{c\in\mC(a,b)}\bigo{\bq_\bp\left(Leaves(c)\right)}+\sum_{c\in\mC(a,b)}\bigo{\mu_{Leaves(c)}}\\
        =\quad&\bigologlogu+\bigo{\sum_{v\in\S\cap[a,b]}\pv}+\bigo{\mu_{\S\cap[a,b]}}\\
        =\quad&\bigologlogu+\bigo{\mu_{\S\cap[a,b]}}+\bigo{\mu_{\S\cap[a,b]}}\\
        =\quad&\bigo{\log\log U+\mu_{\S\cap[a,b]}}
        \end{align*}

        Thus, the expected query time complexity is $\bigo{\log\log U+\mu_{\S\cap[a,b]}}$.


%\header{\bf Modification.} 
% Before introducing the modification operations, we first look into the update cost of the secondary structures caused by the rotation. To explain, to assure the expected $\bigolog$ update cost with the treap, it must be guaranteed  that each rotation causes $\bigo{s}$ update cost if the subtree to be rotated has a size of $s$ as mentioned in theorems for treap (Ref. to Section \ref{sec:treap}). Yet, 
% %the space cost now is $\bigo{n\log^2 n}$ 
% we need to maintain a \textit{right canonical set} and a \textit{left canonical set} for each leaf now 
% and it is unclear if the update cost can be indeed bounded by $O(s)$ after each rotation. Luckily, after careful analysis, we have the following lemma.

% \begin{lemma}\label{os}
% The update cost of the secondary structures caused by a rotation on a subtree of $\T$ with size $s$ is bounded by $\bigo{s}.$
% \end{lemma}
% \begin{proof}
% Without loss of generality, let us consider a right rotation on node $u$ in Figure ?. 
% Without loss of generality, let us consider a right rotation on node $u$ in Figure \ref{fig:treap}. After rotation, only two nodes have a changed slab, i.e., $slab(w)$ changes from $(-\infty,8)$ to $(-\infty,\infty)$, $slab(u)$ changes from $(-\infty,\infty)$ to $[4,\infty)$. After rotation, we swap the \textit{dynamic subset sampling} structures associated with $u$ and $w$, and merge the \textit{dynamic subset sampling} structures associated with $u.left$ and $u.right$ to be the new \textit{dynamic subset sampling} structure of $u$. This cost is bounded by $\bigo{s}$. The \textit{right canonical set} $\mathcal{R}(w,l)$ for each $l\in Leaves(w)$ can be reconstructed as follows: for each $l\in Leaves(w.left)$, we can directly reuse 

% $\mathcal{R}(w,l)$ for each $l\in Leaves(w.left)$ stays unchanged, $\mathcal{R}(w,l)$ for each $l\in Leaves(w.right)$ can be reused after examining if $u.right$ and $w.right.right$ should be added, $\mathcal{R}(w,l)$ for each $l\in Leaves(u.right)$ can be reused after examining if $u.right$ and $u.right.right.right$ should be added. The \textit{right canonical set} $\mathcal{R}(u,l)$ for each $l\in Leaves(w)$ can be constructed as follow: $\mathcal{R}(u,l)$ for each $l\in Leaves(u.right)$ stays unchanged, $\mathcal{R}(u,l)$ for each $l\in Leaves(w.right)$ can be reused after examining if $w.right$ and $w.right.right$ should be added. The construction for the case of the \textit{left canonical set} is analogous.
% Since the cost related to each leaf is constant, the cost of a rotation is $\bigo{s}$.
%\end{proof}

%Now we are ready to introduce the modification operations. 
\header{\bf Modification.} 
For $\instwo{v}{p}$ operation, we insert $v$ into $\T$ in a two-phase manner. We first insert $v$ into $\T$ according to its key value and update the secondary structures of the nodes on the inserting path. 
%since the cost of each node is $\bigone$, the time complexity of the first phase is expected $\bigolog$. 
In the second phase, we may need to rotate up $v$ if the priority generated for it is high. The cost of each rotation at a subtree rooted at $u$ of size $s$ is $f(s)=\bigo{s\log n}$. This is because rotation is a local reconstruction operation, for each  leaf $l$ in $Leaves(u)$ and each ancestor $w$ of $l$, the cost for updating $\mathcal{L}(w,l)$ or $\mathcal{R}(w,l)$ is constant.
%Since our \textit{dynamic subset sampling} structure supports constant time update operations, the cost of a rotation of a subtree of size $s$ in $\T$ is $\bigo{s}$,
% Since during a left rotation or right rotation, there are only two nodes whose slab changes, thus we only need to update the structures associated with these two nodes. The cost of these updates can be made to $\bigo{s}$ by the standard technique of reusing existing structures and doing incremental updates to them.
%According to Claim \ref{os}, the cost of each rotation at subtree of size $s$ is $\bigo{s}$.
Thus according to the theorems for treap in Section \ref{sec:treap}, we know that the expected time necessary to perform an insertion to $\T$ and updating its secondary structures is $\bigo{\frac{n\log n}{ n}+\sum_{i=1}^{n-1}\frac{i\log n}{i^2}}=\bigo{\log n+\log n\sum_{i=1}^{n-1}\frac{1}{i}}=\bigo{\log^2{n}}$. Finally we insert $v$ to the $\VEBT$ and the $\DLCA$, which consumes only $\bigo{\log\log U}$ time. Thus the total insert time is expected $\bigo{\log^2 n}$. 

For the $\delone{v}$ operation, we first rotate $v$ down to the child with greater priority repeatedly until $v$ becomes a leaf, and then remove this leaf. The other steps and analysis for $\delone{v}$ are analogous to $\instwo{v}{p}$ operation.
        
From the above, we can now have the following theorem.
\begin{theorem} \label{rssp2_baseline}
    Given a \textit{dynamic range subset sampling} problem instance $\psi=\left<\S, \bp\right>$, where the keys in $\S$ are integers from $[1,U]$, we can maintain a data structure $\mD$ of size $\mathcal{O}(n\log^2 n)$ with $\bigo{\log\log U+\mu_{\S\cap[a,b]}}$ expected \textbf{query} time if the input range is $[a,b]$. Furthermore, $\mD$ can be dynamically maintained with $\bigo{\log^2 n}$ amortized expected $\upd$, $\ins$ and $\del$ time.
\end{theorem}

==> lemmas/rssp2_final.tex <==

\header{\bf Structure.}
We first apply the size reduction technique three times. Then for each third level chunk $\mC_i$ with size $s=\Theta(\log^2\log\log n)$, we no longer build a baseline data structure for it. Instead, we now build a \emph{dynamic subset sampling} structure for it. Since each chunk consumes only $\bigo{s}$ space, thus in the third level, all the chunks consume $\bigo{\frac{\log^2\log n}{s}s}=\bigo{\log^2\log n}$ space in total. Then a chunk in the second level consume $\bigo{\log^2\log n}$ space, a chunk in the first level consumes $\Bigo{\frac{\log^2 n}{\log^2\log n}\log^2\log n}=\bigo{\log^2 n}$, and the first level chunks consume $\bigo{\frac{n}{\log^2 n}\log^2 n}=\bigon$ space in total.

\header{\bf Query.}
It suffices to show how we sample a subset of third-level chunks on the third level, the operations in the first and second levels are the same as that of Lemma \ref{rssp2_bootstrap}. On the third level, the steps are generally the same as that of Lemma \ref{rssp2_bootstrap}, the slight difference is that we now scan the two marginal nodes to generate a subset. Since we assume that there are no duplicate keys, $n$ is bounded by $\bigo{U}$. As the size of a third level chunk is $\bigo{\log^2\log\log n}=\bigo{\log\log U}$, the scan time of the two marginal nodes is dominated by the term generated by $\VEBT$ and will not increase asymptotic time complexity. Moreover, we only recurse our query three times, which means the time complexity is only multiplied by a constant factor. Thus the final expected time complexity is still $\bigo{\log\log U+\mu_{\S\cap[a,b]}}$

\header{\bf Modification.} 
The modification of the chunks follows the same idea as that of Theorem \ref{rssp_final}.

Finally we have the following theorem.
\begin{theorem} \label{rssp2_final}
    Given a \emph{dynamic range subset sampling} problem instance $\psi=\left<\S, \bp\right>$, where the keys in $\S$ are integers drawn from $[1,U]$, we can maintain a data structure $\D$ of size $\bigon$ with $\bigo{\log\log U+\mu_{\S\cap[a,b]}}$ \textbf{query} time if the input range is $[a,b]$. Furthermore, $\D$ can be dynamically maintained with $\bigo{\log^2 n}$ amortized expected $\upd$, $\ins$ and $\del$ time.
    % Given an $RSSP$ instance $\psi=\left<\S, \bp\right>$, where the values in $\S$ are drawn from grid $[U]$, we can maintain a data structure $\D$ of size $\mathcal{O}(n)$ with $\bigo{\log\log U+\mu_{[a,b]}}$ $\gentwo{a}{b}$ time, furthermore, $\D$ can be dynamically maintained with $\bigolog$ amortized expected $\upd$, $\ins$ and $\del$ time.
\end{theorem}

==> lemmas/rssp2_size_reduction.tex <==

\header{\bf Structure.}
We use the similar chunk idea in Theorem \ref{rssp_final}, but we now set $s$ as an integer between 
%$(\log^2 n-1)$ and $(\log^2 n +1)$. 
$(\log n-1)^2$ and $(\log n +1)^2$. 
We divide $\mR$ into a set of $g=\Theta(\frac{n}{\log^2 n})$ disjoint intervals $\mI_1, ..., \mI_g$ such that each $\mI_i(1\leq i\leq g)$ covers between $\frac{s}{2}$ and $s$ points of $\S$. Then we define $\mC_i=\mI_i\cap\S$ as the $i$-th $chunk$. 

We first create the baseline structure $\mT_{chunk}$ on the chunks using Lemma \ref{rssp2_baseline}. Note the we use $\textbf{q}_\bp(\mC_i)$ as the corresponding probability of the $i$-th $chunk$. This top level structure consumes only $\bigo{g\log g}=\bigo{\frac{n}{\log^2 n}\log^2 \frac{n}{\log^2 n}}=\bigon$ space. However, for each $\mC_i(1\leq i\leq g)$, we no longer solely construct a \emph{dynamic subset sampling} structure as described in Theorem \ref{rssp_final}. Otherwise, we need to scan the marginal chunks containing $a$ and $b$ during query operation, thus increasing the asymptotic time complexity of the query operation. So we build a baseline structure for each $\mC_i$ instead, which takes $\bigo{g s\log^2 s}=\bigo{n\log^2\log n}$ space in total. Now the total space usage is reduced from $\bigo{n\log^2 n}$ to $\bigo{n\log^2\log n}$.

\header{\bf Query.}
Given input range $[a,b]$ at query time, we first locate the chunks $\mC_i$ and $\mC_j$ ($i\leq j$) that contains $a$ and $b$, respectively. Then the points in $\S\cap[a,b]$ are formed by some partial points in $\mC_i$ and $\mC_j$ and all the points in $\mC(i+1,j-1)=\{\mC_{i+1}, \dots, \mC_{j-1}\}$. So we first query $\mT_{chunk}$ with range $[i+1,j-1]$ to get a subset $\mC$, then for each chunk $c\in\mC$, we use the baseline structure associated with it to sample from chunk $c$. Finally, we query the baseline structure of $\mC_i$ and $\mC_j$, respectively. The expected time is
        \begin{align*}
        &\bigologlogu+\bigo{\log\log U+\mu_{\mC_i\cap[a,b]}}+\bigo{\log\log U+\mu_{\mC_j\cap[a,b]}}+\\
        &\bigone+\sum_{c\in\mC(i+1,j-1)}\textbf{q}_\bp\left(Leaves(c)\right)\mathcal{O}(1+\mu_{Leaves(c)})\\
        =\quad&\bigologlogu+\bigo{\log\log U+\mu_{\mC_i\cap[a,b]}}+\bigo{\log\log U+\mu_{\mC_j\cap[a,b]}}+\\
        &\sum_{c\in\mC(i+1,j-1)}\bigo{\textbf{q}_\bp\left(Leaves(c)\right)}+\sum_{c\in\mC(i+1,j-1)}\bigo{\mu_{Leaves(c)}}\\
        =\quad&\bigologlogu+\bigo{\sum_{v\in\S\cap[a,b]}\pv}+\bigo{\mu_{\S\cap[a,b]}}\\
        =\quad&\bigologlogu+\bigo{\mu_{\S\cap[a,b]}}+\bigo{\mu_{\S\cap[a,b]}}\\
        =\quad&\bigo{\log\log U+\mu_{\S\cap[a,b]}}
        \end{align*}

        Thus, the expected query time complexity is $\bigo{\log\log U+\mu_{\S\cap[a,b]}}$.

\header{\bf Modification.} 
    The Modification of the chunks follows the same idea as that of Theorem \ref{rssp_final}.
        
From the above, we can now assert the following lemma.
\begin{lemma} \label{rssp2_bootstrap}
    Given a \emph{dynamic range subset sampling} problem instance $\psi=\left<\S, \textbf{p}\right>$, where the keys in $\S$ are integers drawn from $[1,U]$, we can maintain a data structure $\D$ of size $\mathcal{O}(n\log^2\log n)$ with $\bigo{\log\log U+\mu_{\S\cap[a,b]}}$ \textbf{query} time if the input range is $[a,b]$. Furthermore, $\D$ can be dynamically maintained with $\bigo{\log^2 n}$ amortized expected $\upd$, $\ins$ and $\del$ time.
\end{lemma}

==> lemmas/rssp_baseline.tex <==
        %Before giving our solution, 
        We first introduce the properties of \emph{treap}~\cite{treaps}, an important randomized data structure that will be used in our solution. 
        % Our solution is built upon the \emph{treap}~\cite{treap} data structure. Please see Appendix \ref{intro_treap} for an introduction to \emph{treap} and some related definitions.
        % \begin{definition}[Treap~\cite{treap}]
        %     Given a set $P$ of $n$ items where each item is associated with a \emph{key} and a \emph{priority}. A \emph{treap} for set $P$ is a rooted binary tree $\T$ with node set $P$, arranged in in-order with respect to the keys and in heap-order with respect to the priorities. In-order means that for any node $x$ in the tree, $y.key \leq x.key$ (resp. $y.key \geq x.key$) for all $y$ in the left (resp. right) subtree of $x$. Heap-order means that for any node $x$ with parent $p$, the relation $x.priority < p.priority$ holds.
        % \end{definition}

        %The \emph{treap} data structure has several properties which make it a useful tool for designing nested dynamic data structures.
        \begin{theorem}[properties of treaps~\cite{treap}]
                If $\T$ is a treap for a set $P$ of $n$ items 
                %where the priorities of the items are independent, identically distributed random variables, 
                then the following holds:
                \begin{itemize}[topsep=1mm, partopsep=0pt, itemsep=0pt, leftmargin=14pt]
                %[topsep=1mm, partopsep=0pt, itemsep=0pt, leftmargin=12pt]
                    % \item The expected time  to access an item $x\in P$ in tree $\T$ is $\bigolog$.
                    \item The expected height of $\T$ is $\bigolog$.
                    \item The expected time  to perform an insertion into $\T$ or a deletion from $\T$ is $\bigolog$.
                    \item If the cost of a rotation (including the update cost of secondary structures associated with tree nodes) to a subtree of size $s$ is $\bigo{s}$, then, the expected time needed to update the treap for an insertion or deletion is $\bigolog.$ 
                \end{itemize}      
        \end{theorem}

        \noindent For ease of exposition, we introduce some additional definitions and notations. Let $r$ be the root of $\T$.      
        For a node $u$ in $\T$, we define its $slab$ recursively as follows: 
        % {\em (i)} If $u=r$, then $slab(r)=(-\infty,\infty)$; {\em (ii)} Else, let $p$ be the parent of $u$. If $u$ is the left (resp. right) child of $p$, then $slab(u)=slab(p) \cap \left(-\infty, key(p)\right)$ (resp. $slab(p) \cap [key(p),\infty)$).
        \begin{itemize}[topsep=1mm, partopsep=0pt, itemsep=0pt, leftmargin=14pt]
            \item If $u=r$, then $slab(r)=(-\infty,\infty)$.
            \item Else, let $p$ be the parent of $u$. If $u$ is the left (resp. right) child of $p$, then $slab(u)=slab(p) \cap \left(-\infty, key(p)\right)$ (resp. $slab(p) \cap [key(p),\infty)$).
        \end{itemize}

        \noindent For each node $u\in\T$, we define $Leaves(u)=P\cap slab(u)$. As a well-known fact~\cite{pods22}, for a range $[a,b]$, we can identify a set $\C$ of $\bigo{\log n}$ \emph{canonical nodes} in $\T$ such that: 
        % {\em (i)} The nodes in $\C$ have disjoint subtrees; {\em (ii)} The $Leaves$ in the subtree of the nodes in $\C$ constitute $P\cap[a,b]$.
        \begin{itemize}[topsep=1mm, partopsep=0pt, itemsep=0pt, leftmargin=14pt]
            \item The nodes in $\C$ have disjoint subtrees.
            \item The $Leaves$ in the subtree of the nodes in $\C$ constitute $P\cap[a,b]$.
        \end{itemize}
        We refer the reader to Appendix \ref{appendix:treap} for a more detailed definition of treap and an example that wrap up the concepts mentioned above.
        %\noindent See Appendix \ref{example} for an example of \emph{treap}.
        
        Now we are ready to describe our algorithm.
        % Below are the the description of our algorithm.
        
        \header{\bf Structure.}
        On the top level, we build a \emph{treap} $\T$ on $\S$. The \emph{priority} for each newly inserted treap node is drawn from $\unif{0}{1}$ independently. Thus we can conveniently use the properties of \emph{treap}. For each node $u$ in $\T$, 
        we associate $u$ with a dynamic \emph{subset sampling} structure for $Leaves(u)$ using the data structure in Theorem \ref{sampling structure}.
        Since each value $v$ will be stored in the subset sampling structure of $\bigo{h}$ nodes, and $h$ is $\bigolog$ in expectation, the total space of the structure is thus $\bigo{n\log n}$ in expectation.
            
        \header{\bf Query.}
        Given a input range $[a,b]$ at query time, we answer the query as follows. We first 
            %locate the predecessor (resp. successor) of $a$ (resp. $b$) and 
        find a set $\mC$ of \emph{canonical nodes} for $[a,b]$ in $\bigolog$ time. Suppose $\mC=\setht{u_1, u_2}{u_c}$ for some $c=\bigolog$. 
        %Recap that $Leaves(u_1)$, $Leaves(u_2)$, $\ldots$, $Leaves(u_c)$ are mutually disjoint and their union forms $\S\cap[a,b]$.
        We sample a subset $X_i$ from the dynamic \emph{subset sampling} structure of $u_i$ for $i\in\setht{1}{c}$.
        %The next step is to ask the dynamic \emph{subset sampling} structure of each $u\in\mC$ to generate  a subset, and 
        Finally we return $\cup_{i=1}^{c}X_c$. The overall expected query time is: $$\bigolog+\sum_{i=1}^{c}\bigo{1+\mu_{Leaves(u_i)}}=\bigo{\log n+\mu_{\S\cap[a, b]}}.$$
            
        \header{\bf Modification.}   
        For $\instwo{v}{p}$ operation, we insert $v$ into $\mT$ in a two-phase manner. We first insert $v$ into $\mT$ according to its key value and update the secondary structures of the nodes on the inserting path. Since the cost of updating the secondary structure of each node is $\bigone$, the time complexity of the first phase is expected $\bigolog$. In the second phase, we may need to rotate up $v$ if the priority generated for it is high. Since our dynamic \emph{subset sampling} structure supports constant time modification, the cost of a rotation of a subtree of size $s$ is $\bigo{s}$. Thus according to the properties of treaps, we know that the expected time to perform an insertion to $\mT$ and updating its secondary structures is $\bigolog$. 
    
        For $\delone{v}$ operation, we first rotate $v$ down to the child with greater priority repeatedly until $v$ becomes a leaf and update the secondary structures of the nodes on the path. Finally we remove this leaf. The other steps and analysis for $\delone{v}$ are analogous to $\instwo{v}{p}$ operation.
    
        From this point forward, we will implement $\updtwo{v}{p}$ operation by first performing $\delone{v}$, followed by $\instwo{v}{p}$.

        Now we can derive the following lemma.
        \begin{lemma} \label{rssp_baseline}
            Given a \emph{range subset sampling} problem instance $\psi=\left<\S, \textbf{p}\right>$, we can maintain a data structure $\D$ of size $\mathcal{O}(|\S|\log |\S|)$ with $\mathcal{O}(\log |\S|+\mu_{\S\cap[a,b]})$ expected $\que$ time if the input range is $[a,b]$. Furthermore, $\D$ can be dynamically maintained with $\mathcal{O}(\log |\S|)$ amortized expected $\upd$, $\ins$ and $\del$ time.
        \end{lemma}





==> lemmas/rssp_final.tex <==
        \header{\bf Structure.}
        Let $s$ be an integer between $(\log n - 1)$ and $(\log n + 1)$. We divide $\real$ into a set of $g=\Theta(\frac{n}{\log n})$ disjoint intervals $\mI_1, ..., \mI_g$ such that each $\mI_i(1\leq i\leq g)$ covers between $\frac{s}{2}$ and $s$ elements of $\S$. Then we define $\mC_i=\mI_i\cap\S$ as the $i$-th $chunk$. 
        
        We first create a structure $\mT_{chunk}$ on the chunk level using Lemma \ref{rssp_baseline}. More precisely, the key set is $S_{chunk}=\{1,2,...,g\}$ and the probability function is $\bp_{chunk}(i)=\textbf{q}_\bp(\mC_i)=1-\prod_{v\in\mC_i}(1-\pv)$. The space of $\mT_{chunk}$ is $\bigo{g\log g}=\bigo{\frac{n}{\log n}\log \frac{n}{\log n}}=\bigon$. We also build a dynamic \emph{subset sampling} structure for each $\mC_i(1\leq i\leq g)$ using Theorem \ref{sampling structure}. Note that the sampling probability of each $v\in\mC_i$ should be scaled to $\frac{\bp(v)}{\bp_{chunk}(i)}$. The \emph{subset sampling} structures of all chunks use $\bigo{\sum_{i=1}^g \norm{\mC_i}}=\bigon$ space in total. Thus the overall space consumption of our structure is $\bigon$.
        
        \header{\bf Query.}
        Given input range $[a,b]$ at query time, we answer the \emph{range subset sampling} query as follows. We first locate the intervals $\mI_l$ and $\mI_r$ that contain $a$ and $b$, respectively. If $l=r$, we can answer the query by brute force, i.e., scan $\mC_l=\mC_r$ and decide if each element is sampled or not, this can be done in $\bigolog$ time.

        If $l\neq r$, we can spend $\bigolog$ time to scan the marginal chunks $\mC_l$ and $\mC_r$ to decide if each element is in the range and is sampled or not. For the chunks sandwiched by $\mC_l$ and $\mC_r$, we first query $\mT_{chunk}$ with range $[l+1,r-1]$ to get an index subset $I$. Then, for each $i\in I$, we draw a subset $X_i$ using the \emph{subset sampling} structure of $\mC_i$. Finally, we return $\cup_{i\in I}X_i$. The expected time is:
        \begin{align*}
        &\bigolog+\sum_{i=l+1}^{r-1}\bp_{chunk}(i)\mathcal{O}(1+\frac{\mu_{\mC_i}}{\bp_{chunk}(i)})\\
        =\quad&\bigolog+\sum_{i=l+1}^{r-1}\bigo{\bp_{chunk}(i)}+\sum_{i=l+1}^{r-1}\bigo{\mu_{\mC_i}}\\
        =\quad&\bigolog+\Bigo{\sum_{v\in\S\cap[a,b]}\pv}+\bigo{\mu_{\S\cap[a,b]}}\\
        =\quad&\bigolog+\bigo{\mu_{\S\cap[a,b]}}+\bigo{\mu_{\S\cap[a,b]}}\\
        =\quad&\bigo{\log n+\mu_{\S\cap[a,b]}}.
        \end{align*}
        Thus, the query time complexity is $\bigo{\log n + \mu_{\S\cap[a,b]}}$.
        
        \header{\bf Modification.} 
        $\mT_{chunk}$ is updated whenever the number of points of a chunk changes. This can be done in $\bigo{\log \frac{n}{\log n}}=\bigolog$ time per $\ins\ (\del)$ operation of a point in $\S$. When a chunk overflows (resp., underflows), it can be repaired in $\bigo{s}$ time by chunk split (resp., merge). Using standard amortization analysis, each modification operation only bears $\bigone$ time amortized. Finally, when the size of $\S$ doubles or halves, we rebuild the whole data structure to make sure $s$ is between $(\log n-1)$ and $(\log n  +1)$, and reset $s$ according to the new $n$. Thus the overall modification cost is amortized expected $\bigolog$. %The amortization can be removed by standard techniques(add cite)(DO WE NEED TO REMOVE AMORTIZATION? No need).


        Now we can establish the following theorem.
        \begin{theorem}\label{rssp_final}
            Given a \emph{range subset sampling} problem instance $\psi=\left<\S, \bp\right>$, we can maintain a data structure $\D$ of size $\bigon$ with $\bigo{\log n+\mu_{\S\cap[a,b]}}$ expected $\que$ time if the input range is $[a,b]$. Furthermore, $\D$ can be dynamically maintained with $\bigolog$ amortized expected $\upd$, $\ins$ and $\del$ time.
        \end{theorem}

==> lemmas/wss_geo.tex <==




% \begin{lemma}[jump solution for bounded weight]\label{wss_grs} {
%     Given a \pps~problem instance $\Phi=\left<\S, w\right>$ and a constant $b>0$, if $w(\S)\subseteq(\bar{w}/b, \bar{w}]$, where $\bar{w}\in\real_{>0}$, then after $\bigo{n}$ initialization time, we can create a data structure $\D$ of size $\bigon$ with $\bigo{1}$
%     expected $\que$ time for $\Phi$. Furthermore, $\D$ can be maintained with $\bigone$ $\upd$ time, $\bigone$ expected $\ins$ and $\del$ time. 
% } \end{lemma}


==> lemmas/wss_lookup.tex <==
    \begin{lemma}[table lookup]\label{wss_lookup}
    Suppose $\S^o=\setht{1,2}{m}$ and for all $v\in\S^o$, $w^o(v)$ is greater than $1$ and is bounded by $b^{dm}$, where $d$ is a constant. Then for the \pps~problem instance $\Phi^o= \left< \S^o, w^o \right>$, we can maintain a data structure $\mD^o$ of size $m^{\bigo{m^2}}$ with $\bigone$ expected $\que$ time. Furthermore, $\mD^o$ can be maintained with $\bigone$ $\upd$ time.
    \end{lemma}
    If $m < b$, the above lemma holds trivially. For the remainder of the proof, we will consider the case where $m \geq b$.
    
    To build a lookup table that can correctly answer the query and has small size, we first discretize the weights while ensuring that the sampling probabilities are not scaled down. In the setting of PPS, this is not easily achievable. We explain with the following concrete example.
     \begin{example}
     Suppose $\S^o=\{1,2,3,4\}$, and the weight function is $w(1)=2.9$, $w(2)=7$, $w(3)=3.1$, $w(4)=4.7$. Then we have $\lc w(1)\rc=3$, $\lc w(2)\rc=7$, $\lc w(3)\rc=4$, $\lc w(4)\rc=5$. If we directly sample based on these scaled weights, the probability of $1$ being sampled would become $\frac{3}{3+7+4+5}=\frac{3}{19}$, which is smaller than $\frac{2.9}{2.9+7+3.1+4.7}=\frac{2.9}{17.7}$. Thus we can not directly sample based on the rounded-up weights.
     \end{example}
     To mitigate this problem, we maintain a lookup table with overestimated probabilities, where each element $v$ is sampled with probability $\frac{\lc w^o(v)\rc}{\sum_{v\in\S^o}\lc w^o(v)\rc-m}$ and then apply rejection sampling to correct for the overestimation. Notice that since $m\geq b\geq2$ and for each element $v$ we have $w(v)>1$, $\frac{\lc w^o(v)\rc}{\sum_{v\in\S^o}\lc w^o(v)\rc-m}\leq 1$ is guaranteed.
    
     Next, we are ready to give the detailed proof.
    \begin{proof} 
    The data structure, query operation, and update operation are as follows.
    
    \header{\bf Structure.}
    We define $\bar w(v)=\lc w^o(v)\rc$ for each $v\in\S^o$.
    We use a numeral system with radix $r\triangleq b^{dm}$ to encode $\bar w$, more specifically, $\bar w$ is encoded as:
    $$
    \lambda = \left( \bar w(m)  \bar w(m-1) \ldots \bar w(1) \right)_{r}.
    $$
    Then there are at most $r^m$ possible status of $\bar w$ as $\S^o$ undergoes \upd, i.e., each number in the numeral system with radix $r$ indicates a status of $\bar w$. We also maintain $W=\sum_{i=1}^m w(i)$ and $\overline{W} = \sum_{i=1}^m \lc w(i)\rc$.
    For a given $\bar w$ and a given subset $T$, we want the probability of sampling $T$ from the table to be 
    \begin{align*}
        \bar p(T)=\prod_{v\in T}\frac{\bar w(v)}{\overline{W}-m}\prod_{u\notin T}\frac{\overline{W}-m-\bar w(u)}{\overline{W}-m}\\=\frac{\prod_{v\in T}\bar w(v)\prod_{u\notin T}(\overline{W}-m-\bar w(u))}{(\overline{W}-m)^m}.
    \end{align*}
    % $$\bar p(T)=\prod_{v\in T}\frac{\bar w(v)}{\overline{W}-m}\prod_{u\notin T}\frac{\overline{W}-m-\bar w(u)}{\overline{W}-m}=\frac{\prod_{v\in T}\bar w(v)\prod_{u\notin T}\overline{W}-m-\bar w(u)}{(\overline{W}-m)^m}.$$
    
    Notice that for all subsets $T$ of $\S^o$, their probability sum up to $1$, i.e., $\sum_{T\subseteq \S^o} \bar p(T)=1$. Thus, we can create an array $A_\lambda$ of size $(\overline{W}-m)^m$, where each entry in the array can store a subset. Then we fill $(\overline{W}-m)^m \bar p(T)$ entries of $A_\lambda$ with $T$ for each subset $T$ of $\S^o$. To understand the table, we explain with the following example.
    \begin{example}
        Suppose $\S^o=\{1,2\}$, $b=2$, $d=2$, let us see what should be pre-computed for a specific status of $\bar {w}$, say $\bar w(1)=4,\bar w(2)=3$. First of all, the radix $r=2^{2\times2}=16$, then the $\bar {w}$ is encoded as $\lambda = (3\quad4)_{16}=3\times 16+4\times 1 =52$. We also have $\overline{W}=4+3=7$. Next we create an array $A_{52}$ of size $(\overline{W}-m)^m=(7-2)^2=25$. For subset $\emptyset\subset\S^o$, it is sampled with probability $\frac{7-2-4}{7-2}\times\frac{7-2-3}{7-2}=\frac{2}{25}$, so we fill the first $2$ entry of $A_{52}$ with $\emptyset$. For subset $\{1\}\subset\S^o$, it is sampled with probability $\frac{4}{7-2}\times\frac{7-2-3}{7-2}=\frac{8}{25}$, so we fill the next $8$  entry of $A_{52}$ with $\{1\}$. For subset $\{2\}\subset\S^o$, it is sampled with probability $\frac{7-2-4}{7-2}\times\frac{3}{7-2}=\frac{3}{25}$, so we fill the next $3$ entry of $A_{52}$ with $\{2\}$. For subset $\{1,2\}\subset\S^o$, it is sampled with probability $\frac{4}{7-2}\times\frac{3}{7-2}=\frac{12}{25}$, so we fill the next $12$ entry of $A_{52}$ with $\{1,2\}$. The case when $\bar{w}(1)$ and $\bar{w}(2)$ have other values can be handled by creating new arrays with similarly ways. 
    \end{example}
    As for each $\bar w$, we create an array $A_\lambda$ following the above process. The final space usage is bounded by $r^m\cdot(rm-m)^m\cdot m=m^{\bigo{m^2}}$.
    
    \header{\bf Query.}
    For query, we will look into the array $A_\lambda$ created for the $\bar w$ encoded by $\lambda$. We first uniformly sample an entry from $A_\lambda$, yielding a subset $T$. 
    Because $w(i)>1$, the expectation of the size of the $T$ is 
    $$
    \frac{\sum_{i=1}^m \bar w(i)}{\overline{W}-m}=\frac{\overline{W}}{\overline{W}-m}\leq\frac{2m}{2m-m}=2=\bigo{1}.
    $$
    For each element $v\in T$, we need to apply rejection sampling to correct for the overestimated sampling probability of $\frac{ \bar w(v)}{\overline{W}-m}$. Specifically, for each element $j\in T$, we draw a random number $u$ from $\unif{0}{1}$ and retain $j$ in the final sample if and only if $u<\frac{c\cdot w(v)}{\bar w(v)}\cdot\frac{\overline{W}-m}{W}$. In this way, each element is sampled with probability $\frac{ \bar w(v)}{\overline{W}-m}\cdot\frac{c\cdot w(v)}{\bar w(v)}\cdot\frac{\overline{W}-m}{W}=\frac{c\cdot w(v)}{W}$. Since the expectation of the size of $T$ is $\bigone$, and the rejection step cost $\bigone$ time, the query time is $\bigone$.
    

    
    \header{\bf Update.}
     For $\updtwo{v}{w}$ operation, it is equivalent to updating the $v$-th digit of the $r$-based number $\lambda$, which is a generalized \emph{bit operation}. Specifically, we update $\lambda$ to $$\lfloor\frac{\lambda}{r^v}\rfloor r^v+\lc w\rc r^{v-1}+\lambda\%r^{v-1},$$ which can be done in $\bigone$ time.
    \end{proof}

==> lemmas/wss_naive.tex <==
\begin{lemma} [naive solution] \label{wss_naive} 
    Given a \pps~problem instance $\Phi=\left<\S, w\right>$, after $\bigo{n}$ initialization time, we can create a data structure $\D$ of size $\bigon$ with $\bigon$ $\que$ time for $\Phi$. Besides, $\D$ can be maintained with $\bigone$ $\upd$ time, $\bigone$ expected $\ins$ and $\del$ time.
\end{lemma}
% \begin{proof}
%  We can easily achieve the claimed \upd, \ins~ and \del~ time by maintaining a dynamic array $A$ in arbitrary order and a hash table to map from each element $v\in\S$ to its location in array $A$. Note that in this paper, we implement the standard background rebuilding technique~\cite{rebuilding} to eliminate the amortized cost associated with the rebuilding process. We further maintain the size $n$ of $\S$ and the total weight $W$ of all elements. To answer query, for each $v\in\mS$, we draw a random number $u_v$ from $\unif{0}{1}$. If $u_v < \frac{c\cdot w(v)}{W}$, we include $v$ in $X$. As every element is examined once, the query time is $\bigon$.
%     \vspace{-4mm}
% \end{proof}

==> lemmas/wss_reduce.tex <==
\begin{lemma}[size reduction] \label{wss_sr}
Given a \pps~problem instance $\Phi=\left<\S, w\right>$, 
    assume that using method $\mathcal{M}$, for each non-empty chunk $C$, after linear initialization time, we can create a data structure $\widetilde{\D}(C)$ of linear size for $\Phi_C$ with $\bigo{1}$ $\que$ time and $\bigone$ expected $\upd$ time. Then for the original problem $\Phi$, after $\bigon$ initialization time, we can create a data structure $\mD$ of size $\bigo{n}$ with $\bigo{1}$ expected $\que$ time and $\bigone$ expected $\upd$, $\ins$, and $\del$ time.
\end{lemma}

% The above lemma is proved in Appendix~\ref{pf_wss_sr}.
% \begin{proof}
%     The data structure, query operation and update operations are as follows.

%     \header{\bf Structure.}
%         We keep the biggest weight $w_{max}$ of all the elements, the weights $w(C_t), w^\prime(C_t)$ of each non-empty chunk $C_t$, and the total weight $W$ of all chunks as part of the data structure. 
%         %We use Lemma~\ref{wss_naive} to build a structure $D_{naive}(C_t)$ for each chunk $C_t$, where the elements are ``zeroth-level'' elements.
%         We use method $\mathcal{M}$ to build a structure $\widetilde{D}(C_t)$ for each chunk $C_t$, where the elements are ``first-level'' elements, i.e., buckets.
%         We use Lemma~\ref{wss_grs} to build a structure $D(B)$ for each bucket $B$.
%         We also record the size of $\S$ when we first initialize the data structure in $OldSize$ and record the current size of $\S$ in $Size$. 
%         The total space used is $\bigo{\norm{\S}}+\bigo{\norm{\S}}+\bigo{\norm{\S}}=\bigo{\norm{\S}}$.
    
%     \header{\bf Query.}
%         For query, we first calculate the index of the most significant chunk by $r=\frac{\lc\logb w_{max}\rc}{\lc\logb n\rc}$. Then for each $i\in\{r,r-1,r-2\}$, we first draw a number $u$ from $\unif{0}{1}$, if and only if $u<\frac{w(C_i)}{W}$, we sample subset $Y_i$ from $\widetilde{D}(C_i)$. We further use $D(B)$ to sample from each bucket $B$ in in $Y_i$, and add the sampled elements to the set $X$ to be returned. Then, define $p_{rest}=1-\frac{w(C_r)+w(C_{r-1})+w(C_{r-2})}{W}$. We first draw a number $u$ from $\unif{0}{1}$, if and only if $u<p_{rest}$, we scan each element $v$ in the non-significant chunks and add $v$ to $X$ with probability $\frac{c\cdot w(v)}{W\cdot p_{rest}}$. Finally we return X.
        
%         In this way, each element $v\in R_v\subseteq\C_j$ for $r-2\leq j\leq r$ is sampled into $X$ with probability 
%         \begin{align*}
%             &\frac{w(C_j)}{W}\cdot\frac{w^{\prime}(R_v)}{w^{\prime}(C_j)}\cdot\frac{cw(v)}{w(R_v)}\\
%             =&\frac{w(C_j)}{W}\cdot\frac{w(R_v)}{w^(C_j)}\cdot\frac{cw(v)}{w(R_v)}\\
%             =&\frac{cw(v)}{W}.
%         \end{align*}
%          Each element $v\in\S\setminus C_{sig}$ is sampled into $X$ with probability $p_{rest}\cdot \frac{c\cdot w(v)}{W\cdot p_{rest}}=\frac{c\cdot w(v)}{W}$.

%         The expected time complexity is:
%         \begin{align*}
%         &\sum_{i=r-2}^{r}\bigo{1}+\sum_{C\in C_{sig}}\frac{w(C)}{W}\bigo{1}+p_{rest}\Bigo{\left|\S\setminus C_{sig}\right|} \\
%         \leq\quad&\bigone+\sum_{v\in\S}\frac{w(v)}{W}\bigone+\frac{1}{\norm{\S}}\bigo{\norm{\S}}\\
%         =\quad&\bigo{1}+\bigone+\bigone \\
%         =\quad&\bigo{1}.
%         \end{align*}
%     \header{\bf update.}
%         We need to reconstruct the whole data structure every time the size doubles or halves since last construction. The amortized cost for construction is $\bigone$. If a update operation does not incur reconstruction, its cost is also $\bigone$ because it changes at most two chunks.
% \end{proof}
\begin{proof}
      The data structure, along with the query and update algorithms, are explained individually as follows.

    \header{\bf Structure.}
        We first scan $\S$ to put each element into its corresponding bucket. We then scan again to put each bucket into its corresponding chunk.
        We utilize method $\mathcal{M}$ to construct a structure $\widetilde{D}(C)$ for each non-empty chunk $C$.
        %, where the elements are ``first-level'' elements, specifically bucket IDs.
        Additionally, we employ Lemma~\ref{wss_grs} to build a structure $D(B)$ for each bucket $B$. We also store several pieces of information as part of the data structure. This includes 
        %the largest weight $w_m$ among all elements, 
        the weights $w(C_t)$ and $w^\prime(C_t)$ for each non-empty chunk $C_t$, and the total weight $W_\S$. We also keep track of the initial size of $\S$ when initializing the data structure as $OldSize$, and the current size of $\S$ as $Size$. Given that the structures for each subproblem require linear space and initialization time, the total space and initialization time for the entire problem is $\bigo{n}$.
    
    \header{\bf Query.}
        To answer a query, we first find the largest ID of non-empty chunk $r$. Let $x=\frac{\lc\logb W\rc}{\lc\logb n\rc}$. It is easy to verify that the following should hold: $x-2\leq r\leq x$; otherwise, it is impossible for the total weight of the $n$ elements to be $W$. Then, we can easily check if $C_x$, $C_{x-1}$, $C_{x-2}$ is empty in order to identify the largest ID of non-empty chunk.
        %if there exists element with ID larger than $r$ (resp. smaller than $r$), then the weight will be larger (resp. smaller) than $W$, resulting in a contradiction. 
        Next, for each $i\in\{r-2,r-1,r\}$, we draw a random number $u$ from the uniform distribution $\unif{0}{1}$. If $u<\frac{w(C_i)}{W}$, we sample a subset $Y_i$ from the structure $\widetilde{D}(C_i)$, which takes $\bigone$ time according to the property of $\mathcal{M}$. We further utilize the structure $D(B_j)$ to sample elements from bucket $B_j$ for each ID $j$ in $Y_i$, adding the sampled elements to the set $X$ to be returned. This step also takes $\bigone$ time according to Lem~\ref{wss_grs}. Next, we define $p_{\text{rest}}=1-\frac{w(C_{r-2})+w(C_{r-1})+w(C_{r})}{W}$. We draw a random number $u$ from the uniform distribution $\unif{0}{1}$. If $u<p_{\text{rest}}$, we scan each element $v$ in the non-significant chunks and add $v$ to $X$ with probability $\frac{c\cdot w(v)}{W\cdot p_{\text{rest}}}$. Finally, we return $X$.
        
        Under this sampling scheme, each element $v\in B^v\subseteq\C_i$ for $r-2\leq i\leq r$ is sampled into $X$ with probability 
        \begin{align*}
            &\frac{w(C_i)}{W}\cdot\frac{w^{\prime}(B^v)}{w^{\prime}(C_i)}\cdot\frac{c\cdot w(v)}{w(B^v)}=\frac{w(C_i)}{W}\cdot\frac{w(B^v)}{w(C_i)}\cdot\frac{c\cdot w(v)}{w(B^v)}=\frac{c\cdot w(v)}{W}.
        \end{align*}
         Each element $v\in\S\setminus C_{sig}$ is sampled into $X$ with probability $p_{rest}\cdot \frac{c\cdot w(v)}{W\cdot p_{rest}}=\frac{c\cdot w(v)}{W}$.

        The expected time complexity is:
        \begin{align*}
        &\sum_{i=r-2}^{r}\bigo{1}+\sum_{C\in C_{sig}}\frac{w(C)}{W}\bigo{1}+p_{rest}\Bigo{\left|\S\setminus C_{sig}\right|} \\
        \leq\quad&\bigone+\sum_{v\in\S}\frac{w(v)}{W}\bigone+\frac{1}{\norm{\S}}\bigo{\norm{\S}}\\
        =\quad&\bigo{1}+\bigone+\bigone = \bigo{1}.
        \end{align*}
\header{\bf Update.}
        We need to reconstruct the entire data structure every time the size of the set $\S$ doubles or halves since the last construction. The amortized cost for reconstruction is $\bigone$. Recap that we can implement the background rebuilding technique for the rebuilding process, thus this amortized cost can be eliminated. If an update operation does not incur reconstruction, its cost is also $\bigone$ because it changes only one chunk and one bucket for \ins~ and \del~ and at most two chunks and two buckets for \upd.  Thus, it only takes constant time to update these information. Also, it only takes constant time to update $W$ and $Size$.
\end{proof}

